AlphaSparse: Generating High Performance SpMV Codes Directly from Sparse Matrices

Sparse Matrix-Vector multiplication (SpMV) is an essential computational kernel in many application scenarios. Tens of sparse matrix formats and implementations have been proposed to compress the memory storage and speed up SpMV performance. We develop AlphaSparse, a superset of all existing works that goes beyond the scope of human-designed format(s) and implementation(s). AlphaSparse automatically \emph{creates novel machine-designed formats and SpMV kernel implementations} entirely from the knowledge of input sparsity patterns and hardware architectures. Based on our proposed Operator Graph that expresses the path of SpMV format and kernel design, AlphaSparse consists of three main components: Designer, Format \& Kernel Generator, and Search Engine. It takes an arbitrary sparse matrix as input while outputs the performant machine-designed format and SpMV implementation. By extensively evaluating 843 matrices from SuiteSparse Matrix Collection, AlphaSparse achieves significant performance improvement by 3.2$\times$ on average compared to five state-of-the-art artificial formats and 1.5$\times$ on average (up to 2.7$\times$) over the up-to-date implementation of traditional auto-tuning philosophy.

==> src/back.tex <==

\subsection{Sparse Matrix Formats}

In recent decades, dozens of sparse matrix formats have been designed artificially by researchers for diverse design goals including compressing memory storage space, reducing memory access, improving load balance, reducing thread divergence for GPUs, etc.
These formats store only non-zero elements and ignore zeros which take a major portion of a sparse matrix.
(Refer to the work \cite{langr2015evaluation} and \cite{filippone2017sparse} for good summaries of them).
We categorize sparse matrix formats into three groups: Root Formats, Derived Formats, and Hybrid Formats.

Four of them are generally considered as basic formats \cite{li2013smat, filippone2017sparse, xie2019ia}, or \emph{Root Formats} in this paper, which consists of COOrdinate (COO), Compressed Sparse Row (CSR), ELLPACK (ELL), and DIAgonial (DIA).
The COO format stores row and column indices along with the value of every non-zero;  
The CSR format further compresses row indices by only storing starting positions of each row;
The ELL format eliminates row indices by padding the non-zeros of each row to the same length, thus only padded column indices and values are stored. 
The DIA format has some specialties from the above due to the dense or padded diagonal pattern shown in a sparse matrix, thus it saves diagonal offsets and their values. 

To handle more irregular matrices, better memory compression, or higher performance of sparse kernels, plenty of artificially \emph{Derived Formats} have been proposed.
We refer to a derived format as a format manually designed based on only ONE root format,  such as Blocked COORdinate (BCOO)~\cite{im2004sparsity}, derived from COO; CSR5~\cite{liu2015csr5}, derived from CSR; Sliced ELLPACK (SELL), derived from ELL, to name a few. 

Beyond root and derived formats, the third category is \emph{Hybrid Formats} which flexibly use multiple formats for different portions of a sparse matrix.
It could be a mix among root formats or a mix of root and derived formats, such as HYBrid (HYB), COCKTAIL \cite{su2012clspmv}, and  Compressed Sparse eXtended (CSX) \cite{kourtis2011csx}. 

% In this work, we will focus on COO, CSR, and ELL root formats, their derived ones due to their better popularity.



% To reduce memory access overhead, formats of sparse matrix only store non-zero elements (nz/nzs). In recent 40 years, dozens of format is proposed by human for different design goals, like reducing memory access, increasing load balance, reducing thread divergence, etc. \cite{langr2015evaluation} and \cite{filippone2017sparse} summarize mainstream sparse matrix formats of recent years. The most basic formats are COO, ELL, CSR. COO includes row index, col index for each nz. CSR further compresses row index of COO by just storing index of row's first nz. ELL even eliminates row index by padding the nz of each row to the same number. To handle more irregular matrices, their derived formats are also proposed, like SELL, BCOO \cite{im2004sparsity}, CSR5 \cite{liu2015csr5}, etc. 

% Unlike formats mentioned before, some hybrid formats are also proposed in recent years, which use different formats in different parts of matrix, like HYB, clSpMV \cite{su2012clspmv}, CSX \cite{kourtis2011csx}, etc. 

% \begin{figure}[htbp] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
% \centering
% \includegraphics[width=0.46\textwidth]{search_space.pdf} 
% \caption{Example of formats and kernels may be ignored by existing human's works}
% \label{CompareSearchSpace} %用于文内引用的标签
% \end{figure}



\subsection{Motivations} \label{motivation}

The motivation of \nickname{} comes from three observations below. 

\textit{Observation 1: Artificial formats and their sparse kernel algorithms are limited by human's experience and narrow search space.}
%  due to large step sizes
Newly proposed artificial sparse matrix formats and auto-tuners have covered increasingly more sparse patterns, however, they are limited by human's experience and a narrow search space. 
A new format, either a derived or hybrid format, is generally created based on a root format, a previously derived format, or is a mixture of several root or derived formats. 
For example, the CSR5 format is derived from the root format CSR; while the hybrid format HYB is derived from two root formats COO and ELL, illustrated in \Cref{CompareSearchSpacesize}(a).
Since the new format design is limited by the designer's experience on data compression and sparse algorithm implementation, which makes proposing the optimal format for a given sparse matrix becomes a very difficult task and an NP-hard problem counting the kernel algorithms and their parameters in \Cref{CompareSearchSpacesize}(b).
\Cref{CompareSearchSpacesize}(a) shows three example cases which have been ignored by existing format and SpMV kernel designs but are discovered by our \nickname{}.
Case 1 uses the existing row-grouped CSR \cite{oberhuber2010new} format but with a new implementation by combining thread level reduction of CSR5 \cite{liu2015csr5} and global memory reduction of row-grouped CSR implementations. 
Case 2 introduces a new format by combining the indices reduction of CSR-Adaptive~\cite{greathouse2014efficient} and the blocking strategy of row-grouped CSR, while reusing CSR-Adaptive's kernel implementation. 
Case 3 proposes both new format and its new corresponding kernel implementation by using binning strategy of ACSR~\cite{ashari2014fast} but the ELL format in each bin.


% Although existing auto-tuners can cover more matrix sparse patterns, they are limited by human's experience and narrow search space. As shown in Figure \ref{CompareSearchSpace}, assuming there are m formats have been proposed by human. And each format may have multiple kernel implements (like CSR), assuming number of kernels is n (n >= m). Even though all of them are included in auto-tuner, the search space size is n. However, huge search space between different artificial formats, different kernel implements as well as their combination is ignored. This space includes a large amount of "theoretically existing formats or kernel implements" that mix human works' philosophies. For example, Figure \ref{CompareSearchSpace} includes three representative cases which may be ignored by some mainstream SpMV designs in figure. Case1 includes format of CSR5 and new kernel implement strategy combining thread level reduction of CSR5 and global memory reduction of row-grouped CSR. Case2 includes CSR-Adaptive's kernel implement strategy and new format combining reduction index of CSR and blocking strategy of row-grouped CSR. Case3 includes both new format and kernel implement strategy. It includes binning strategy of ACSR, and uses ELL in each bin. If we take these new formats, new kernel implement strategies as well as new combinations of kernel and format into consideration, the ideal search space can be greatly expanded. Assuming new format space size is M (M > m) and new kernel space size is N (N > n), the total search space size is M $\times$ N, which is much larger than n.

\begin{figure}[htbp] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering
\includegraphics[width=0.48\textwidth]{hybrid_design_example.pdf} 
\caption{Mixed designs found by \nickname{} on the matrix \emph{2D\_27628\_bjtcai}}
\label{MixtheDesigns} %用于文内引用的标签
\end{figure}

\begin{figure*}[htbp] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering
\includegraphics[width=0.9\textwidth]{total_overview.pdf} 
\caption{Overview of AlphaSparse.}
\label{AlphaSparseOverview} %用于文内引用的标签
\end{figure*}

\textit{Observation 2: New formats and implementations could be automatically created to achieve higher performance of sparse kernels.}
We have seen newly automatically created formats and/or kernel implementations by \nickname{} from the three cases.
\Cref{MixtheDesigns} shows the performance of two mixed designs found by our \nickname{} derived from three formats and their implementations on an example sparse matrix \emph{2D\_27628\_bjtcai} from SuiteSparse Matrix Collection~\cite{10.1145/2049662.2049663}. 
The CSR-Adaptive format \cite{greathouse2014efficient} achieves 39 GFLOP/s on its corresponding SpMV kernel; while the row-grouped CSR format \cite{heller2012adaptive} gets 58 GFLOP/s and the bottom Sliced ELL (SELL) format~\cite{kreutzer2012sparse} performs 61 GFLOP/s on its counterparts.
While by combining blocking strategy of row-grouped CSR with reduction strategy of CSR-Adaptive, the performance of the mixed format is 75 GFFLOP/s, higher than that of either of the two formats.
Similarly, by mixing the format and implementations from the blocking of SELL and Row-Grouped CSR and the reduction of CSR-Adaptive, the performance could be even higher as 95 GFLOP/s.
These two mixed format and implementation designs have been ignored by the existing work but could be discovered by \nickname{} with higher SpMV performance.

% The second observation is that by mixing the design of existing formats and kernels, new format can be created and sometimes it can provide higher performance. Figure \ref{MixtheDesigns} shows the design of three formats for \emph{2D\_27628\_bjtcai} in SuiteSparse Matrix Collection. The first format is row-grouped CSR \cite{heller2012adaptive}. It divides each row into chunks which are mapped to threads, and it reduces intermediate results from chunks in global memory. Its performance is 25 gflops. The third format is CSR-Adaptive \cite{daga2015structural}, which maps each nz to thread and reduces the intermediate results of them in shared memory. Its performance is 38 gflops. By combining blocking strategy of row-grouped CSR with reduction strategy of CSR-Adaptive, performance of mixed format is 62 gflops.


\begin{figure}[htbp] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering
\includegraphics[width=0.46\textwidth]{Graph_of_SELL.pdf} 
\caption{The steps of converting a tiny sparse matrix in COO format to Sliced ELL (SELL) format. Blue blocks are non-zeros, while blank ones are zeros.}
\label{CovertCOOFormatMatrixtoSELL} %用于文内引用的标签
\end{figure}



\textit{Observation 3: Sparse formats are convertible to each other with common steps, making creating a new format feasible from a source artificial format.}
This observation has been proved by other work~\cite{chou2020automatic}, although they emphasized on the conversion among existing artificial formats.
Usually, when a new artificial format is designed, the conversion stage will be provided as well from another popular source artificial format, such as CSR or COO format~\cite{filippone2017sparse}.
We take the conversion from COO to SELL with four steps as an example, shown in \Cref{CovertCOOFormatMatrixtoSELL}. 
Beginning from the dense representation with zeros, all non-zeros are first pushed to the left side of the matrix; then the rows are sorted in a decreasing order; then the matrix is blocked by rows with relatively similar lengths gathered in a block; finally the rows of each block are padded to the maximum length. 
The four steps are commonly existed in other format conversions.
The conversion from COO to Blocked ELL~\cite{barbieri2015three, choi2010model} has the same three steps except the "Sort" step; while if further removing the "Block Row" step, then the output format is ELL.
Thus, it is feasible by taking common conversion steps as building blocks to convert or even create a format automatically.
\nickname{} chooses the COO format as the universal source format to start the conversion process to any other formats due to its simplicity.

% Then, the matrix is blocked by rows and the row sizes of each block is padded to the same. The conversions of different formats are common and can be reused. If "Sort" is not included, the output format would be blocked-ELL. And if "Row Block" is further removed, the output format would be ELL. The first observation shows that by describing how a format is converted from COO, we can get a fine-grained model for representing matrix formats.




The three observations above make automatically generating sparse representation and its SpMV implementation on demand and achievable only based on the knowledge of the input sparse matrix. 
% These two observations show that, because of a fine-grained model and higher performance of new mixed format, creating better format by machine is necessary and feasible.

==> src/design-space.tex <==

% \todo{move the following context to introduction. In this part, we should explain "expression"' why/what/how in several words.}
% which describes how both SpMV formats and kernels are designed. 
To unify the format and kernel design space, AlphaSparse proposes a fine-grained model, the \textit{Operator Graph}. An Operator Graph is an expression of the "path" to a specific coordinate or position of the format-kernel design space, which takes a sparse matrix stored in the Matrix Market file format as input, and provides the SpMV code at the end of the path as output.
In this section, we will introduce \textit{Designer} of AlphaSparse, which constructs and executes the Operator Graph and prepares matrix metadata for the following process.

\subsection{Operator}

Given a sparse matrix, we summarize that an SpMV code is generally developed in three steps: 1) defining a compressed memory layout (i.e., format) of the matrix partly as a data structure in the code, and converting the matrix to this representation;
2) mapping (distributing) it to hardware units; % programming model
% 2) mapping non-zero elements to hardware units and further converting matrix, 
3) designing kernel implementation, mainly SpMV reduction strategies. 
AlphaSparse follows these stages {\it converting}, {\it mapping} and {\it kernel}. 
Each of the three stages consists of multiple common operations or optimization strategies, which we call \textit{operators} to represent expert knowledge in our Operator Graph model.
% During the course of the three stages, there are some common operations among data layout conversions and kernel implementations. 
% We call them operators  in modeling.

% As mentioned in Figure \ref{CovertCOOFormatMatrixtoSELL} and Section \ref{motivation}, the design of the format is derived from the format converting operations with commonality. In the philosophy of AlphaSparse, these "operations" are not limited in format conversion, but expanded to kernel implement (shown in \ref{KernelCodeGenerator}), so called Operator. Operator is expert knowledge-based modeling to express a pattern of SpMV format and kernel design.

% As shown in Table \ref{TheExampleofFormatDesignNode}, Operators are from three stages of operator graph: converting stage, mapping stage, kernel stage. These three stages correspond to three steps in SpMV format design: 1) defining a memory data layout of matrix, 2) mapping non-zero elements to hardware computing resource and further converting matrix, 3) designing kernel implement, mainly includes SpMV reduction strategy, for corresponding format.

We list the operators in \nickname{} in \Cref{TheExampleofFormatDesignNode} along with their sources and descriptions.
Almost all of them are derived from existing research as shown in the "Source" column. 
In this work, we only consider operators for GPUs as a prototype.

Operators in converting stage are for sparse format definition.
"ROW/COL\_DIV" divides the whole matrix into striped sub-matrices in row or column direction. 
"SORT", "SORT\_SUB" and "BIN" reorder rows of the matrix according to row size. DENSE\_DECOM and DIA\_DECOM separate the locally dense parts or diagonal band parts from the original matrix \cite{su2012clspmv}. 
"COMPRESS", the last operator in converting stage, pushes non-zeros to the left of each row, like the arrangement in the ELL format without zero padding.
% "COMPRESS" make the following operators ignore zeros of each row and it would finish converting stage. 

Mapping stage begins after "COMPRESS" operator. 
Operators suffixed by "\_BLOCK" cut adjacent non-zeros of the matrix into blocks and map them to different levels of parallelism.
% (i.e, thread grid of CUDA). 
The other operators in this stage further trims the memory layout inside of blocks.

Operators in kernel stage
\footnote{Since "WARP\_SEG\_ADD\_RED" and "THREAD\_BITMAP\_RED\_G" are added by us, no source citation for them.}
not only contribute to format, but also determine how kernels are implemented. 
"SET\_RESOURCE" sets the structure of the thread grid when launching a GPU kernel. Operators suffixed by "\_RED" means different reduction strategies for intermediate results of BMTB, BMW, or BMT in an SpMV Kernel. 
Most of the operators contain different types of parameters. For example, "ROW/COL\_DIV" has its parameter as an array to define the row or column partitioning positions;
% indices where a matrix is divided. 
"BMT\_NNZ\_BLOCK" has an integer parameter to define the number of non-zeros of each BMT. 
We consider the operators critical to SpMV performance in this work are also derived from formats like HYB, CSB \cite{bulucc2009parallel}, etc. Users can add their own operators.

Dependencies exist between some operators. Some dependencies come from operators' semantics. For example, operators prefixed with "BMW" and "BMT" cannot be followed by operators prefixed with "BMTB". Because when a data block has already mapped to a group of threads or warps, it cannot be split and mapped to a thread block, due to the structure of the thread grid and GPU hardware architecture. And others can also be defined by users for search pruning. 


% are impossible to be mapped to thread block.  according to the grid setting. 
% Dependencies can also be defined by users for search pruning. 
% AlphaSparse also provides some interfaces for this.


% Operator is the basic element of Operator Graph, which includes logic of matrix metadata modification. Table \ref{TheExampleofFormatDesignNode} shows some examples of operators. And almost all of them are derived from existing formats, which are shown in column "Source" of Table \ref{TheExampleofFormatDesignNode}. For more detailed example, ROW\_DIV is a operator in converting stage. It divides the whole matrix into several submatrices. This operator would cause bifurcations of the graph and each branch would launch a SpMV kernel. BMTB\_ROW\_BLOCK is a operator in mapping stage. It cuts the matrix from the row direction, and maps each row band to GPU thread block. GBL\_ATOM\_RED is a operator in kernel stage. It uses atomic add to reduce intermediate results of the same row in global memory.

\subsection{Operator Graph}

By connecting operators in order, Operator Graph combines a series of design patterns and finally determines the design path to generate an SpMV code. It is the key data structure of AlphaSparse. It is generated by Search Engine (Section \ref{SearchEngine}) of AlphaSparse. Beginning with the input node, operators which can satisfy the dependencies with graph existing operators would be randomly chosen and connected behind. When no operator can satisfy the dependencies, the graph generation would finish. Designer would execute the complete graph by executing its operators in orders, which include logic to modify Matrix Metadata Set (shown in \ref{KernelCodeGenerator}). Matrix Metadata Set includes all current matrix states. It is the basis for format and kernel generation. 

The upper part of Figure \ref{ExampleofEnumeratingGraph} shows how to generate an Operator Graph for an input matrix. The generation of this graph begins with an operator (operator 1) inputting a matrix. And operators satisfying dependencies would be randomly chosen and connected at the end of the existing graph. In this case, the operator named "ROW\_DIV" (operator 2) cuts the matrix into three row bands and uses different designs for different parts. After the complete graph is generated, Designer executes these operators in order by modifying Matrix Metadata Set, which is prepared for format and kernel generation.


==> src/intro.tex <==
Sparse Matrix-Vector multiplication (SpMV) is one of the most computational kernels in many domains, such as climate simulation, material science, molecular dynamics, data analytic \cite{chen2018gflink, kyrola2012graphchi}, machine/deep learning \cite{wang2019deep, zhang2016cambricon}, to name a few. 
In the past decades, a large amount of formats \cite{ashari2014efficient, langr2015evaluation,filippone2017sparse, ashari2014fast, maggioni2013adell, heller2012adaptive, yan2014yaspmv, liu2018towards, kreutzer2012sparse, liu2015csr5, greathouse2014efficient} have been proposed to efficiently compress sparse matrices in memory on diverse hardware architectures including x86 multi-core CPUs, many-core Graphics Processing Units (GPUs) \cite{owens2008gpu}, Intel Xeon Phi accelerators \cite{sodani2016knights}, and Field-Programmable Gate Array (FPGAs) \cite{kuon2008fpga}.
Along with the development of sparse matrix formats, improvements in SpMV kernel implementations are flourishing.


%The number of possible solutions%
\begin{figure*}[htbp] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering
\includegraphics[width=0.95\textwidth]{search_space_size.pdf} 
\caption{Three-dimensional space of SpMV code design (b), truncated artificial format-kernel space (a), and our \nickname{}'s design principle in format-kernel space (c). }
% Search space of traditional auto-tuner based on format selection, and AlphaSparse based on SpMV design pattern. (a) is projection of design space on the surface bounded by format space and kernel space. (b) is design space of SpMV program. (c) is search space of existing auto-tuner based on format selection. 
\label{CompareSearchSpacesize} %用于文内引用的标签
\end{figure*}


% describe the problem -- design space
Since sparse formats and SpMV kernel implementations depend on the appearance of an input matrix and the underneath computer architectures, we use a three-dimensional space to represent the design space which consists of formats, implementations, and optimization parameters to describe the huge number of choices to generate an SpMV code for a given sparse matrix.
This design space is enormous though not continuous because: 1) the three dimensions are not continuous by nature. 
For example, two arbitrary sparse matrix formats could have very small differences by one or multiple arrays in their data structures, but this difference is discrete. 
2) The three-dimensional design space is not continuous as well, since a given format could be coupled with multiple SpMV implementations, and implementation could include multiple parameters and their ranges as spaces.
Thus, we use dots in \Cref{CompareSearchSpacesize}(b) to represent the enormous discrete design space.
% \jli{Add the space size calculation?}
Exploring the design space could fulfill two traditional goals: \textit{new SpMV code design}, consisting of a format and its SpMV implementation; and \textit{the optimal SpMV code search} based on existing formats and implementations.

% As shown in Figure \ref{CompareSearchSpace}, assuming there are m formats have been proposed by human. And each format may have multiple kernel implements (like CSR), assuming number of kernels is n (n >= m). Even though all of them are included in auto-tuner, the search space size is n. If we take these new formats, new kernel implement strategies as well as new combinations of kernel and format into consideration, the ideal search space can be greatly expanded. Assuming new format space size is M (M > m) and new kernel space size is N (N > n), the total search space size is M $\times$ N, which is much larger than n.

% During the past 40 years, Sparse Matrix Vector multiplication (SpMV) has become one of the most important kernel in many domains, including scientific computing  \cite{vazquez2010improving,xiao2019caspmv}, data analytic \cite{chen2018gflink, kyrola2012graphchi}, machine learning \cite{wang2019deep, zhang2016cambricon}, etc. To improve SpMV performance, in the past few years, a large amount of matrix storage formats \cite{ashari2014efficient, langr2015evaluation,filippone2017sparse, ashari2014fast, maggioni2013adell, heller2012adaptive, yan2014yaspmv, kreutzer2012sparse, liu2015csr5, greathouse2014efficient} have been proposed on the recent hardware architectures such as many-core Graphics Processing Units (GPUs). 

% design new format
\textbf{\textit{New SpMV code design.}}
We give a small set of formats and SpMV kernel implementations (blue circles and squares) in \Cref{CompareSearchSpacesize}(a) to illustrate the relationship between them.
Most of the formats have a corresponding kernel implementation, e.g., all formats except CSR format in this figure. 
Even though from a theoretical view, one format could have multiple implementations due to the usage of architectural features and porting to diverse architectures.
While few formats, particularly popular ones, have been designed with more than one kernel implementation by far, e.g., the CSR format has "Stream" and "Vector" implementations~\cite{ashari2014fast}.
This phenomenon shows that \textit{format and kernel spaces in existing designs are not orthogonal but coupled, which largely narrows the design space} in \Cref{CompareSearchSpacesize}(b). 

% existing auto-tuners does not cover searching this huge design space
\textbf{\textit{The optimal SpMV code search.}}
To pursue the optimal solution, i.e. the best SpMV performance, in this tremendous design space, 
% Because of irregular sparsity of matrix, a format or kernel implement designed by human can't provide high SpMV performance in all matrices. 
quite some auto-tuning frameworks \cite{li2013smat, zhao2018bridging, benatia2016sparse, zhao2018overhead, nisa2018effective, niu2021tilespmv, su2012clspmv, kourtis2011csx} have been proposed to search for the "optimal" format and kernel implementation from a small group of artificial formats.
% provide much higher average performance across all matrices. 
% All these works select a best artificial format for specific matrix. 
SMAT~\cite{li2013smat} and the work~\cite{zhao2018bridging} select from Coordinate (COO), Compressed Sparse Row (CSR), ELLPACK/ITPACK (ELL), and DIAgonal (DIA) formats; ClSpMV~\cite{su2012clspmv} takes DIA, CSR, ELL and their blocked derivation as candidates formats for submatrices to construct a hybrid format;
CSX~\cite{kourtis2011csx} designs and chooses from various patterns for tiny submatries.
% SMAT \cite{li2013smat} selects the best format from COO, CSR, ELL and DIA. ClSpMV, TileSpMV and CSX preprocess the matrix before format selection. TACO \cite{kjolstad2017tensor} selects how index is compressed (CSR or CSC) in each dimension for high-order tensors, which essentially selects from CSR and CSC (or other existing formats) in 2-dimension matrix.
By comparing to \Cref{CompareSearchSpacesize}(b), \emph{these auto-tuners consider a very small range of formats and limited kernel implementations and parameters correspondingly}.
Besides, the search strategies of the optimization problems in these auto-tuners generally have clear steps: firstly finding the "optimal" format; then searching the "optimal" kernel implementation of that format; finally determining the parameter values when the format and kernel implementation have been fixed~\cite{balaprakash2011can}.
This strategy's exploration paths are parallel with the three axes, straightforwardly reducing the exploration to a combinatorial search problem, shown as the blue lines in \Cref{CompareSearchSpacesize}(c) when projected to the format-kernel space.
\emph{This kind of search strategies neglect immense design space.}

% \tgm{A traditional auto-tuner first starts from a fixed format and find out its optimal kernel by searching a huge parameter space. Then it turns to another format and search again until the best combination of format and kernel is selected. Unlike the traditional way that straightforwardly reduces to a combinatorial search problem, AlphaSparse expresses the optimization space as an {\tt operator graph} that simulates the design philosophy of human while exploiting much larger space than human. That is, {\tt operator graph} is an expression of the "path" to specific position of design spaces, which describes how both SpMV formats and kernels are designed in a extremely fine-grained way. }

% As shown in Figure \ref{CompareSearchSpacesize}(b), the origin problem of SpMV auto-tuning is searching the best combination of format, kernel and their parameters, which so called finding the optimal solution in design space. 
% Existing auto-tuners simply treat this problem as selecting the best format and corresponding kernel from existing artificial formats and kernels, shown in Figure \ref{CompareSearchSpacesize}(c). 
% To directly creating SpMV formats and kernel, AlphaSparse further reduces search step size by regarding the problem of SpMV auto-tuning as combinatorial optimization of SpMV design patterns. 


\nickname{} not only achieves the two traditional goals simultaneously by directly exploring the original three-\\dimensional space, but could generate codes even beyond the scope of existing artificial formats and kernels and is smarter than existing auto-tuners with much larger search space.
AlphaSparse expresses the projected format-kernel design space in \Cref{CompareSearchSpacesize}(c) using \textit{Operator Graphs} that simulates the design philosophy of human to exploit much larger space.
An Operator Graph is the "path" to a specific position of the design space, which describes the very fine-grained design procedure of an SpMV code, both the sparse format and its SpMV implementation.
The red arrows paths in \Cref{CompareSearchSpacesize}(c) represent Operator Graphs in a simple way.
% are vectors representing design patterns.
It takes a sparse matrix as input, determines the direction and step size of each step considering input features, and creates an optimal and high performance SpMV code  consisting of matrix format and kernel implementation, the end point of a path in the figure.
% The essence of \nickname{}'s SpMV code design is equal to stepping to the specific position in design space by superposing vector of design patterns. 

Different from the existing research that the Operator Graph could explore the whole design space which includes but far beyond the found artificial formats (e.g., CSR and ELL marked as blue dots in the red path in \Cref{CompareSearchSpacesize}(c)).
The state-of-the-art work either 1) creates artificial format and kernel design by firstly finding the "optimal" format in only the format space direction, then determine its best kernel implementation (the blue path in \Cref{CompareSearchSpacesize}(c)); or 2) searches the "optimal" SpMV code in a small set of existing artificial formats and implementations in their auto-tuners.
% After the optimal solution is found, the best format, kernel as well as parameter can be get by projecting it to these three spaces.


% Figure \ref{CompareSearchSpacesize}(a) is projection of design space on the surface bounded by format space and kernel space, red arrows are vectors representing design patterns. 
% In AlphaSparse, the essence of SpMV program design is equal to stepping to the specific position in design space by superposing vector of design patterns.
% To solve the problem of auto-tuning based on format selection, this paper proposes AlphaSparse. 
% AlphaSparse proposes \textbf{Operator Graph}, a new way to model sparse matrix format by expressing design of format. 
% It describes how a format is generated from origin COO matrix step by step. 
% By mixing Operator Graphs of nearby artificial formats and kernels, AlphaSparse can further search the space between existing SpMV program designs. 

AlphaSparse has three main components: Designer, Format \& Kernel Generator, and Search Engine, to accomplish design space's expression, projection, and exploration. Designer and Format \& Kernel Generator accept Operator Graph as input, and generate format as well as corresponding kernel code according to it. Search Engine aiming at finding an Operator Graph with high performance. While searching, SpMV performance corresponding to Operator Graph can be get by directly running generated SpMV code.

We implement AlphaSparse by nearly 90,000 lines of C++ code and evaluate it with several state-of-the-art and high-performance artificial formats on NVIDIA GPUs. AlphaSparse largely improves SpMV performance by up to 8.5$\times$ (2.06$\times$ on average) compared to state-of-the-art five human-designed formats. 
We also compare AlphaSparse with the best SpMV performance using brute-force auto-tuning search among the five formats.
% to mimic the behavior of auto-tuners but in 100\% accuracy.
% philosophy based on format selection. 
% By comparing SpMV performance with the best artificial formats of specific test matrices,
AlphaSparse still achieves up to 2.59$\times$ (1.35 $\times$ on average) performance improvement. 
The code of \nickname{} will be released. 

Our main contributions are summarized as follows:
\begin{itemize}
    \item We first introduce the whole three-dimensional design space of the SpMV code generation problem, which also categorizes and maps existing work to the space. (\Cref{background})
    \item We develop \nickname{}, which is easy-to-use by taking matrix-market files as input and outputs an optimal and high performance SpMV code. (\Cref{overview})
    % \item We propose a new auto-tuning philosophy based on format creating. This philosophy helps AlphaSparse break through the limitation of artificial formats.
    \item We propose new graph-based modeling, named Operator Graph, to express the design space. (\Cref{formatdesigner})% for the design of matrix format and SpMV kernel.
    \item We design format and template-based kernel projectors to generate compressed data representation and high performance implementation. (\Cref{KernelCodeGenerator} )
    \item We adopt guided search on Operator Graphs and pruning to find the optimal SpMV code with competitive performance. (\Cref{SearchEngine})
    % a fine-grained searching process based on a combinatorial optimization problem, which can further search the space between existing SpMV program designs.
    \item We evaluate AlphaSparse on 915 large matrices from SuiteSparse Matrix Collection and obtain three counter-intuitive insights produced by machine. (\Cref{evaluation})
\end{itemize}

% The rest of the paper is organized as follows. Section \ref{background} presents several storage formats of sparse matrices, existing auto-tuning frameworks and our motivation. In Section \ref{overview} we propose an overview of AlphaSparse. Then we describe the three core features: format designer, kernel code generator and search engine in Section \ref{formatdesigner}, Section \ref{KernelCodeGenerator} and Section \ref{SearchEngine}. In Section \ref{evaluation} we evaluate AlphaSparse and show some insights of sparse matrix format design. Related work is presented in Section \ref{relatedworks}, and conclusion is in Section \ref{conclusionandfuturework}.

==> src/model-driven-format-compression.tex <==
% \subsection{Model-Driven Format Compression}
% \label{ModelDrivenFormatCompression}

% The performance of the kernel that is directly generated from the template is much lower than the hand-writing kernel. Format \& Kernel Generator of AlphaSparse includes many optimizations for IR, such as removing unnecessary features, removing unnecessary loops, combining multiple short-data-type features with into one, etc. \textit{Model-Driven Format Compression is a key optimization provided by AlphaSparse, which makes the idea of this work feasible.} Because SpMV is a memory-bottleneck \cite{davis2012spmv} kernel, reducing the memory usage of the final matrix format can reduce memory access and improve performance. \textit{This optimization accomplishes this goal by transforming array type data (in memory) to models and replacing memory access with calculation. The compression can eliminate up to 50\% memory access, compared with rough kernel code.}

% Figure \ref{ExampleofMemoryAccessOptimization} shows that an array from format can be eliminated by transforming it into a model. In this case, an operator named BMTB\_ROW\_DIV divides the matrix into row bands every 64 lines, and each row band is mapped to a thread block. It adds an array to the format, which includes the first row index of BMTB for thread-block-level reduction. 

% Without optimization, this index needs to be read from global memory (row\_offset=reduce\_row\_offset\_arr[bid]). But by fitting array index and value to a linear model, this index can be calculated directly by index of BMTB (row\_offset=64*bid), without any memory access. In the manual kernel implementation, skilled engineer can discover the simple patterns of format array and directly write the optimized code, sometimes even unconsciously. AlphaSparse performs this optimization explicitly. In addition to linear function, as shown in Figure \ref{ExampleofMemoryAccessOptimization}, some other functions, like step function and periodic linear function, are also supported. Absolutely, hypothesis function of model can also be extended.

% Unlike normal regression problems for data analysis, models in our optimizer must guarantee 100\% accuracy. Any error in models would cause wrong SpMV implementation. To improve the success rate of this optimization, a small number of errors in the model can be tolerated. AlphaSparse would add if statements to the kernel and separately assign values for the specific array index that the model cannot fit. Because branches in SIMT hardware cause thread divergence, we set a threshold of 12 for the number of allowed errors or branches.

==> src/overview.tex <==

AlphaSparse is developed to directly generate the optimal machine-designed SpMV code (program), by utilizing matrix design philosophy from existing artificial format and kernel designs but in a fine-grained model. Different from traditional auto-tuning and artificial format design works, which treat matrix formats and kernels independently, \nickname{} considers the format and kernel spaces simultaneously. Thus, in \nickname{}, designing new code and searching for the optimal code in given formats are unified as one search problem for the optimal solution in the large design space. 
AlphaSparse accepts a sparse matrix in matrix-market file format as input and outputs the best format and SpMV kernel implementation (SpMV code) for this matrix. The optimal SpMV code can be directly leveraged to accelerate users' applications.

Sparsity and irregularity make the performance of the SpMV program sensitive to input matrix patterns. To solve this, AlphaSparse proposes a fine-grained model, named \textit{Operator Graph}, which describes and explores the format and kernel space together. The Operator Graph expresses the path in the design space (see \Cref{CompareSearchSpacesize}(c)) with a single operator for each step. An operator combines the kernel strategy and format design into a unified expression. New formats and kernels are created through traversing an Operator Graph. 

AlphaSparse consists of an \textit{Search Engine} (\Cref{SearchEngine}) for finding a path to the optimal solution in the design space, a \textit{Designer} (\Cref{formatdesigner}) to execute the design patterns in this path, and a \textit{Format \& Kernel Generator} (\Cref{KernelCodeGenerator}) which projects the design patterns % the point of design space
to format and kernel implementation, shown in \Cref{AlphaSparseOverview}. The Search Engine starts enumerating Operator Graphs by traversing all possible graph structures depending on user-defined node/operator dependencies and the corresponding parameter configurations for every node, under a given search strategy.
% After Enumerator enumerating structure and parameters of graph, 
A complete Operator Graph generated by the enumerator each time will be sent to the Designer. 
% The example Operator Graph in \Cref{AlphaSparseOverview} shows the three stages of a sparse matrix being converted from the original representation of matrix-market file by passing a serial of operators (graph nodes) in order. 
Designer executes operators of graph in order and records operators' cumulative effect on the input matrix in Matrix Metadata Set, which includes all of details of the current matrix. After the Operator Graph is executed, Format \& Kernel Generator generates kernel code and format according to the kernel design stage 
% (more details are shown in Section \ref{formatdesigner} 
of the Operator Graph and matrix final states in Matrix Metadata Set, with several optimization methods, especially Model-Driven Format Compression.
% (in Section \ref{KernelCodeGenerator}), the generated kernel provides competitive performance with human-written codes. 
% By compiling and directly running the generated SpMV kernel, 
The SpMV performance will be recorded after compiling and running the generated code from a particular Operator Graph, and further interpolated by AI to a more fine-grained cost model.
Till the termination condition is satisfied, the Search Engine outputs the optimal SpMV code according to the cost model.
% and the tuning process will return to Search Engine.
% , getting performance of SpMV kernels corresponding to them, and 
% And graph enumeration is limited by node (operator) dependency and search strategy (step size of node parameter search) of Enumerator.

% In addition to getting format performance by directly running kernel of format, performance can also be fast predicted by machine learning model 

AlphaSparse provides a simple interface to users. Users just need to input a matrix in matrix-market file format. And an Operator Graph, a final optimal format, a kernel implementation can be got. Also, an Operator Graph can be used as a format conversion routine and a code design guideline for a specific input pattern. Although AlphaSparse provides much higher performance than human's design, users can further optimize it by modifying the output Operator Graph or implementing a more efficient format conversion routine.
% Extensibility is also important in AlphaSparse's design. In AlphaSparse, Operators of graph can be created by users by implementing some interfaces and configuring node dependency, which reduces the structure search step size of the format space. 

In the following sections, we will discuss the three main components: Designer, Format \& Kernel Generator, and Search Engine.
% And they will show how a optimal matrix format and corresponding kernel code is generated by machine. 
